Data Augmentation for Image Classification using Generative AI

Scaling laws dictate that the performance of AI models is proportional to the amount of available data. Data augmentation is a promising solution to expanding the dataset size. Traditional approaches focused on augmentation using rotation, translation, and resizing. Recent approaches use generative AI models to improve dataset diversity. However, the generative methods struggle with issues such as subject corruption and the introduction of irrelevant artifacts. In this paper, we propose the Automated Generative Data Augmentation (AGA). The framework combines the utility of large language models (LLMs), diffusion models, and segmentation models to augment data. AGA preserves foreground authenticity while ensuring background diversity. Specific contributions include: i) segment and superclass based object extraction, ii) prompt diversity with combinatorial complexity using prompt decomposition, and iii) affine subject manipulation. We evaluate AGA against state-of-the-art (SOTA) techniques on three representative datasets, ImageNet, CUB, and iWildCam. The experimental evaluation demonstrates an accuracy improvement of 15.6% and 23.5% for in and out-of-distribution data compared to baseline models, respectively. There is also a 64.3% improvement in SIC score compared to the baselines.

==> case_study.tex <==
\section{A Motivating Case Study}
\label{sec:case_study}


Text-to-image, image-to-image, and inpainting are three key image augmentation techniques extensively utilized in recent image augmentation works. We conducted a case study of these methods for several datasets like ImageNet~\citep{deng2009imagenet}, CUB~\citep{wah2011caltech}, and iWildCam~\citep{koh2021wilds}, to understand their advantages and shortcomings. We discuss our observations using a representative image of a bird from the CUB data set, as illustrated in Figure~\ref{fig:casestudy}. 


\noindent{\bf Text-to-image:} It can be observed that text-to-image, while capable of generating a high diversity of images, often produces samples in which the subject is so drastically altered that even human observers struggle to identify it. We find in the figure that the identifying mark of the bird, the red ring around the neck, is missing in the augmented images, which would translate into failures for downstream tasks.

\noindent{\bf Image-to-image:} This type of augmentation frequently results in a significant loss of subject detail, akin to the image-to-text method. We see that the bird is very hard to spot in the augmented image, which might make the downstream object detection task tougher. The prairie chicken in the example appears to have been transformed into a parrot.

\noindent{\bf Inpainting:} This method operates by modifying the image within a masked area based on a text prompt, yet this method can inadvertently corrupt the subject's appearance. We see that the orange/red identifying ring misplaced in one of the augmented images, thus this method can corrupt the subject. 

 In contrast, our proposed approach does not add any artifacts to the subject image. It successfully generates augmented images with diverse backgrounds while preserving the authenticity of the subject as seen in the augmented images by \name. This form of data augmentation has the potential to translate into better performance in terms of fine-grained classification, generalizability, and explainability. Our proposed approach is presented in the next section.
 \vspace{-10pt}


==> src_limitations.tex <==
\section{Limitations}
\label{sec:limitation}

Though \name focuses on generating augmented images in data scarcity scenarios, it fails several times to generate images with visual consistency. Our framework faces challenges in compatibility issues between the augmented image subjects and their backgrounds. Figure~\ref{fig:imagenet10_results}
and additional results in the supplementary materials sometimes display unnatural images. Moreover, although the augmented image generation process is a one-time task, it requires a resource-intensive pipeline involving several tools, such as diffusion models, segmentation models, and others.

